Domain Name System Security and Privacy: A Contemporary Survey

The domain name system (DNS) is one of the most important components of today's Internet, and is the standard naming convention between human-readable domain names and machine-routable IP addresses of Internet resources. However, due to the vulnerability of DNS to various threats, its security and functionality have been continuously challenged over the course of time. Although, researchers have addressed various aspects of the DNS in the literature, there are still many challenges yet to be addressed. In order to comprehensively understand the root causes of the vulnerabilities of DNS, it is mandatory to review the various activities in the research community on DNS landscape. To this end, this paper surveys more than 170 peer-reviewed papers, which are published in both top conferences and journals in the last ten years, and summarizes vulnerabilities in DNS and corresponding countermeasures. This paper not only focuses on the DNS threat landscape and existing challenges, but also discusses the utilized data analysis methods, which are frequently used to address DNS threat vulnerabilities. Furthermore, we looked into the DNSthreat landscape from the viewpoint of the involved entities in the DNS infrastructure in an attempt to point out more vulnerable entities in the system.

==> bios.tex <==


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ak}}]{Aminollah Khormali} is a PhD student at the Department of Computer Science at the University of Central Florida. He has obtained his Master's of Science degree in Mechatronics Engineering from the K. N. Toosi University of Technology, in Tehran, Iran, in 2015. At UCF, he is a member of the Security and Analytics Lab (SEAL), where he is working in the area of computer and network systems security. In particular, he explores the science of detecting and analyzing large-scale vulnerabilities in the context of network systems, IoT, cryptocurrency, and deep learning. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ha}}]{Hisham Alasmary} is a PhD student at the Department of Computer Science at the University of Central Florida. He has obtained his Master's of Science degree in Computer Science from The George Washington University, in Washington, D.C., USA, in 2016. At UCF, he is a member of the Security and Analytics Lab (SEAL), where he is working in the area of computer and network systems security. In particular, he explores the science and practice of threat information sharing and IoT security. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{aa}}]{Afsah Anwar} 
 is a PhD student at the Department of Computer Science at the University of Central Florida. He has obtained his Bachelors of Technology degree in Electronics and Communication Engineering from the Jamia Millia Islamia (JMI), in New Delhi, India, in 2014. At UCF, he is a member of the Security and Analytics Lab (SEAL), where he is working in the area of computer systems security. He builds automation tools for analyzing and mitigating vulnerabilities and their lifecycles in the context of large-scale software systems, mobile systems, and IoT. 
% I augment my work by a predictive angle to the vulnerability ecosystem, cost, and lifecycles.

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{jc}}]{Jinchun Choi} 
is a PhD student at the Department of Computer Science at the University of Central Florida and the Department of Computer Information Science of Inha University (joint PhD program). He has obtained his B.Eng. and M.S. degrees in Computer \& Information Engineering from the Inha University, in Incheon, Korea, in 2011, 2014, respectively. He is a member of the Global Research Lab on Big Data Security and is conducting research in the field of information security. In particular, his interests include biometrics, machine learning, network security, user authentication, and IoT security.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{jmp}}]{Jeman Park} 
is a Ph.D. student at the Department of Computer Science at the University of Central Florida and a member of the Security and Analytics Lab (SEAL). He obtained his B.Sc. degree in Computer and Communication Engineering from Korea University, in Seoul, South Korea, in 2016. His work has been focused on privacy, DDoS detection and mitigation, DNS security, anonymous network (Tor), and IoT security. He is a member of IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/grayscale_saad}}]{Muhammad Saad} is a PhD. student in the Department of Computer Science at the University of Central Florida. He obtained his Bachelor's degree in Electrical Engineering from National University of Sciences and Technology (NUST) in 2014. He completed his Masters in Electrical Engineering from Lahore University of Management Sciences (LUMS) in 2017. At UCF, Saad is a member of the Security Analytics and Research Lab (SEAL) advised by Prof. Aziz Mohaisen. His research spans blockchain technology with emphasis on the attack surface of blockchains. His work has appeared in reputable venues including ASIACCS 2018 and HotPOST 2018.
\end{IEEEbiography}

\if0
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{dn}}]{DaeHun Nyang}
received a B.Eng. degree in electronic engineering from Korea Advanced Institute of Science and Technology, and M.S. and Ph.D. degrees in computer science from Yonsei University, Korea in 1994, 1996, and 2000 respectively. He has been a senior member of the engineering staff at Electronics and Telecommunications Research Institute, Korea, from 2000 to 2003. Since 2003, he has been an associate professor at the Computer Information Engineering Department of Inha University, Korea where he is also the founding director of the Information Security Research Laboratory. He is a member of the board of directors and an editorial board of Korean Institute of Information Security and Cryptology. Dr. Nyang's research interests include cryptography and network security, privacy, usable security, biometrics and their applications to authentication and public key cryptography.
\end{IEEEbiography}
\fi

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Awad}}]{Amro Awad} 
is an Assistant Professor at the Department of Electrical and Computer Engineering at the University of Central Florida (UCF). Before joining UCF and right after he received his Ph.D. from North Carolina State University, he was a Senior Member of Technical Staff at Sandia National Laboratories in Albuquerque, NM. He was also selected as  Summer Faculty Fellow with the U.S. Air Force in their Cyber Assurance Branch. His research focus is on secure hardware architectures and hardware/software co-design. His research publications have been published in top-venues such as ISCA, ASPLOS, HPCA, PACT and ICS.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{az}}]{Aziz Mohaisen} 
is an Associate Professor at the Department of Computer Science at the University of Central Florida. He obtained his Ph.D. from the University of Minnesota in 2012, was an Assistant Professor at SUNY Buffalo, a Senior Scientist at Verisign Labs, and a Research Engineer at ETRI. At UCF, he directs the Security and Analytics Lab (SEAL), where he works in the broad area of computer security and privacy with applications to malware detection, distributed denial of service, critical infrastructure, Internet of Things, and blockchain systems. He was awarded the Summer Faculty Fellowship from the US AFOSR (2016) and several best paper awards (IEEE ICDCS 2017, WISA 2014, and CNS 2013). He is an Associate Editor of IEEE Transactions on Mobile Computing (TMC) and has been on the organizing committee of various top conferences; he was recognized for his service to IEEE INFOCOM (2017 and 2018) and IEEE CNS (2016). His work has been supported by NSF, NRF, AFRL, AFOSR, and FC2, appeared in major conferences and journals, and was featured in MIT Technology Review, the New Scientist, Scientific American, Financial Times, Science Daily, Slashdot, The Verge, Deep Dot Web, and Slate, among others. He is a Senior Member of ACM (2018) and IEEE (2015).

\end{IEEEbiography}
